Local right biadjoints, bistable pseudofunctors and 2-geometries for Grothendieck topoi

We provide bicategorical analogs of several aspects of the notion of geometry in the sense of the theory of spectrum. We first introduce a notion of local right biadjoint, and prove it to be equivalent to a notion of bistable pseudofunctor, categorifying an analog 1-categorical result. We also describe further laxness conditions, giving some properties of the already known lax familial pseudofunctors. We also describe 2-dimensional analogs of orthogonality and factorization systems, and use them to construct examples of bistable pseudofunctors through inclusion of left objects and left maps. We apply the latter construction to several examples of factorization systems for geometric morphisms to produce geometry-like situations for Grothendieck topoi. In particular we prove a new (terminally connected, pro-etale) factorization theorem for geometric morphisms, which corresponds to a certain local geometry involved in the general construction of spectra.

==> Lax_stable_inclusion_from_lax_generic_bifactorization_system.tex <==
\subsection{Lax-stable inclusion from lax-generic bifactorization}

Lax bifactorization systems were named so because of the analogy of their lefts maps with the lax generic morphisms. Here we detail how those two notion are related. However one should carefully note that we must add the assumption of left full-faithfulness of the bifactorization system in order to get all the desired property of the lax stables functors. 


\begin{theorem}
Let be $ (\mathcal{L, \mathcal{R})}$ a left full and faithful, pseudofunctorial, lax generic bifactorization system on a 2-category $ \mathcal{C}$. Then we have a lax stable inclusion
\[  \mathcal{C}^\mathcal{R} \hookrightarrow \mathcal{C}  \]
where $ \mathcal{C}^\mathcal{R}$ is the (0,2)-full sub-2-category consisting of all objects of $\mathcal{C}$, $\mathcal{R}$-maps between them, and no restrictions on 1-cells. Moreover its lax generic 1-cells are exactly the $\mathcal{L}$-maps - and they are pseudofunctorial. 
\end{theorem}

\begin{proof}
We must first prove that the left maps are exactly the lax generic, but this is immediate: indeed the diagonalization property of the lax generic induces in particular that the diagonalization of pseudocommutative squares left to a right maps have invertible left and rights part in the generic diagonalization: hence lax generic are automatically in $\mathcal{L}$ as they are left bi-orthogonal to any right maps; conversely, lax genericity is exactly what is required for a factorization system to have its left maps lax generic relatively to this inclusion. Pseudofunctoriality of lax generic 1-cells is entailed from the pseudofunctoriality of the lax generic bifactorization system. \\

Now any arrow $ f : A_1 \rightarrow A_2$ in $\mathcal{C}$ has a $(\mathcal{L},\mathcal{R})$ factorization 
% https://q.uiver.app/?q=WzAsMyxbMCwwLCJBXzEiXSxbMiwwLCJBXzIiXSxbMSwxLCJBX2YiXSxbMCwxLCJmIl0sWzAsMiwibF9mIiwyXSxbMiwxLCJyX2YiLDJdLFsyLDMsIlxcYWxwaGFfZiBcXGF0b3AgXFxzaW1lcSIsMSx7InNob3J0ZW4iOnsidGFyZ2V0IjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dXQ==
\[\begin{tikzcd}
	{A_1} && {A_2} \\
	& {A_f}
	\arrow[""{name=0, anchor=center, inner sep=0}, "f", from=1-1, to=1-3]
	\arrow["{l_f}"', from=1-1, to=2-2]
	\arrow["{r_f}"', from=2-2, to=1-3]
	\arrow["{\alpha_f \atop \simeq}"{description}, Rightarrow, draw=none, from=2-2, to=0]
\end{tikzcd}\]
We must prove this factorization to be a lax generic 2-cell. If $ \alpha_f$ factorizes as
%Suppose one has a factorization of $\alpha_f$ as below, with $r$ in $\mathcal{R}$:
% https://q.uiver.app/?q=WzAsMyxbMCwwLCJBXzEiXSxbMSwwLCJBXzIiXSxbMCwxLCJBX2YiXSxbMCwyLCJuX2YiLDJdLFswLDEsImYiXSxbMiwxLCJyIiwxXSxbMiwxLCJyX2YiLDIseyJjdXJ2ZSI6Mn1dLFs1LDAsIlxcVXBhcnJvdyBcXHNpZ21hICIsMSx7InNob3J0ZW4iOnsic291cmNlIjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFs2LDUsIlxceGkiLDIseyJzaG9ydGVuIjp7InNvdXJjZSI6MjAsInRhcmdldCI6MjB9fV1d
\[\begin{tikzcd}[sep=large]
	{A_1} & {A_2} \\
	{A_f}
	\arrow["{n_f}"', from=1-1, to=2-1]
	\arrow["f", from=1-1, to=1-2]
	\arrow[""{name=0, anchor=center, inner sep=0}, "r"{description}, from=2-1, to=1-2]
	\arrow[""{name=1, anchor=center, inner sep=0}, "{r_f}"', curve={height=18pt}, from=2-1, to=1-2]
	\arrow["{\Uparrow \sigma }"{description}, Rightarrow, draw=none, from=0, to=1-1]
	\arrow["\xi"', shorten <=2pt, shorten >=2pt, Rightarrow, from=1, to=0]
\end{tikzcd}\]
Then we have two alternative factorizations of the same invertible lax square 
% https://q.uiver.app/?q=WzAsNCxbMCwwLCJBXzEiXSxbMSwwLCJBXzIiXSxbMCwxLCJBX2YiXSxbMSwxLCJBXzIiXSxbMCwyLCJsX2YiLDJdLFswLDEsImYiXSxbMiwxLCJyIiwxXSxbMiwzLCJyX2YiLDJdLFsxLDMsIiIsMCx7ImxldmVsIjoyLCJzdHlsZSI6eyJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzYsMCwiXFxVcGFycm93IFxceGkiLDEseyJzaG9ydGVuIjp7InNvdXJjZSI6MjB9LCJzdHlsZSI6eyJib2R5Ijp7Im5hbWUiOiJub25lIn0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbNyw2LCJcXFVwYXJyb3cgXFx4aSIsMSx7InNob3J0ZW4iOnsic291cmNlIjoyMCwidGFyZ2V0IjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dXQ==
\[\begin{tikzcd}[sep=large]
	{A_1} & {A_2} \\
	{A_f} & {A_2}
	\arrow["{l_f}"', from=1-1, to=2-1]
	\arrow["f", from=1-1, to=1-2]
	\arrow[""{name=0, anchor=center, inner sep=0}, "r"{description}, from=2-1, to=1-2]
	\arrow[""{name=1, anchor=center, inner sep=0}, "{r_f}"', from=2-1, to=2-2]
	\arrow[Rightarrow, no head, from=1-2, to=2-2]
	\arrow["{\Uparrow \sigma}"{description}, Rightarrow, draw=none, from=0, to=1-1]
	\arrow["{\Uparrow \xi}"{description}, Rightarrow, draw=none, from=1, to=0]
\end{tikzcd} = \begin{tikzcd}[sep=large]
	{A_1} & {A_2} \\
	{A_f} & {A_2}
	\arrow["{l_f}"', from=1-1, to=2-1]
	\arrow["f", from=1-1, to=1-2]
	\arrow[""{name=0, anchor=center, inner sep=0}, "{r_f}"{description}, from=2-1, to=1-2]
	\arrow["{r_f}"', from=2-1, to=2-2]
	\arrow[Rightarrow, no head, from=1-2, to=2-2]
	\arrow["{\alpha_f \atop \simeq}"{description, pos=0.7}, Rightarrow, draw=none, from=0, to=1-1]
\end{tikzcd}\]
But from $ \alpha_f$ is invertible, the left one is the universal filler obtained by orthogonality up to a canonical invertible 2-cell. Hence, by the universal property of the factorization of lax square as detailed in \cref{factorization of lax square in lax fact system}, there exists a unique $ \zeta : r \Rightarrow r_f$ such that $\sigma$ decomposes as
% https://q.uiver.app/?q=WzAsMyxbMCwwLCJBXzEiXSxbMCwxLCJBX2YiXSxbMSwwLCJBXzIiXSxbMCwxLCJsX2YiLDJdLFswLDIsImYiXSxbMSwyLCJyX2YiLDFdLFsxLDIsInIiLDIseyJjdXJ2ZSI6M31dLFs1LDAsIlxcYWxwaGFfZiBcXGF0b3AgXFxzaW1lcSIsMSx7ImxhYmVsX3Bvc2l0aW9uIjo3MCwic2hvcnRlbiI6eyJzb3VyY2UiOjIwLCJ0YXJnZXQiOjIwfSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzYsNSwiXFx6ZXRhIiwyLHsic2hvcnRlbiI6eyJzb3VyY2UiOjIwLCJ0YXJnZXQiOjIwfX1dXQ==
\[\begin{tikzcd}[sep=large]
	{A_1} & {A_2} \\
	{A_f}
	\arrow["{l_f}"', from=1-1, to=2-1]
	\arrow["f", from=1-1, to=1-2]
	\arrow[""{name=0, anchor=center, inner sep=0}, "{r_f}"{description}, from=2-1, to=1-2]
	\arrow[""{name=1, anchor=center, inner sep=0}, "r"', curve={height=18pt}, from=2-1, to=1-2]
	\arrow["{\alpha_f \atop \simeq}"{description, pos=0.7}, Rightarrow, draw=none, from=0, to=1-1]
	\arrow["\zeta"', shorten <=3pt, shorten >=3pt, Rightarrow, from=1, to=0]
\end{tikzcd}\]
Now the condition of lax-generic concerning parallel 2-cells is ensured by the condition that $( \mathcal{L},\mathcal{R})$ is a left full and faithful bifactorization system, so that parallel 2-cells between $\mathcal{R}$-maps that are equified by a $\mathcal{L} $-map are equal.\\

Now observe that for $ l$ in $\mathcal{L}$ and $r $ in $\mathcal{R}$, if the identity $ 1_{rl}$ factorizes as 
% https://q.uiver.app/?q=WzAsMyxbMCwwLCJBXzEiXSxbMCwxLCJBXzIiXSxbMSwwLCJBXzMiXSxbMCwxLCJsIiwyXSxbMCwyLCJybCJdLFsxLDIsInInIiwxXSxbMSwyLCJyIiwyLHsiY3VydmUiOjN9XSxbNSwwLCJcXFVwYXJyb3cgXFxzaWdtYSIsMSx7InNob3J0ZW4iOnsic291cmNlIjoyMH0sInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFs2LDUsIlxceGkiLDIseyJzaG9ydGVuIjp7InNvdXJjZSI6MjAsInRhcmdldCI6MjB9fV1d
\[\begin{tikzcd}
	{A_1} & {A_3} \\
	{A_2}
	\arrow["l"', from=1-1, to=2-1]
	\arrow["rl", from=1-1, to=1-2]
	\arrow[""{name=0, anchor=center, inner sep=0}, "{r'}"{description}, from=2-1, to=1-2]
	\arrow[""{name=1, anchor=center, inner sep=0}, "r"', curve={height=18pt}, from=2-1, to=1-2]
	\arrow["{\Uparrow \sigma}"{description}, Rightarrow, draw=none, from=0, to=1-1]
	\arrow["\xi"', shorten <=3pt, shorten >=3pt, Rightarrow, from=1, to=0]
\end{tikzcd}\]
then in particular the 2-cell 
% https://q.uiver.app/?q=WzAsNCxbMCwwLCJBXzEiXSxbMSwxLCJBXzIiXSxbMiwwLCJBXzMiXSxbMSwwLCJBXzIiXSxbMCwxLCJsIiwyXSxbMSwyLCJyJyIsMV0sWzAsMywibCJdLFszLDJdLFsxLDMsIlxcVXBhcnJvdyBcXHNpZ21hIiwxLHsic2hvcnRlbiI6eyJzb3VyY2UiOjIwfSwibGV2ZWwiOjIsInN0eWxlIjp7ImJvZHkiOnsibmFtZSI6Im5vbmUifSwiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dXQ==
\[\begin{tikzcd}
	{A_1} & {A_2} & {A_3} \\
	& {A_2}
	\arrow["l"', from=1-1, to=2-2]
	\arrow["{r'}"{description}, from=2-2, to=1-3]
	\arrow["l", from=1-1, to=1-2]
	\arrow[from=1-2, to=1-3]
	\arrow["{\Uparrow \sigma}"{description}, Rightarrow, draw=none, from=2-2, to=1-2]
\end{tikzcd}\]
must be reflected by left full-faithfulness by a 2-cell $ \zeta : r' \Rightarrow r$ such that $ \sigma$ factorizes as
% https://q.uiver.app/?q=WzAsMyxbMCwwLCJBXzEiXSxbMCwxLCJBXzIiXSxbMSwwLCJBXzMiXSxbMCwxLCJsIiwyXSxbMSwyLCJyIiwxXSxbMSwyLCJyJyIsMix7ImN1cnZlIjozfV0sWzAsMiwicmwiXSxbNCwwLCI9IiwxLHsic2hvcnRlbiI6eyJzb3VyY2UiOjIwfSwic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoibm9uZSJ9LCJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzUsNCwiXFx6ZXRhIiwyLHsic2hvcnRlbiI6eyJzb3VyY2UiOjIwLCJ0YXJnZXQiOjIwfX1dXQ==
\[\begin{tikzcd}
	{A_1} & {A_3} \\
	{A_2}
	\arrow["l"', from=1-1, to=2-1]
	\arrow[""{name=0, anchor=center, inner sep=0}, "r"{description}, from=2-1, to=1-2]
	\arrow[""{name=1, anchor=center, inner sep=0}, "{r'}"', curve={height=18pt}, from=2-1, to=1-2]
	\arrow["rl", from=1-1, to=1-2]
	\arrow["{=}"{description}, Rightarrow, draw=none, from=0, to=1-1]
	\arrow["\zeta"', shorten <=3pt, shorten >=3pt, Rightarrow, from=1, to=0]
\end{tikzcd}\]
and we shall have that $ 1_{r'} = \xi\zeta$ for $ l$ equifies those 2-cells. Hence equality 2-cells of the form $ 1_{rl}$ are generic. \\


Now we must prove the composition condition for lax generic 2-cells. 

\end{proof}
